Disruptive Forces in Metamaterial Tweezers for Trapping 20 nm Nanoparticles Based on Molecular Graphene Quantum Dots

In recent years, plasmonic optical tweezers have been used to trap nanoparticles and study interactions with their environment. An unavoidable challenge is the plasmonic heating due to resonant excitation and the resulting temperature rise in the surrounding environment. In this work, we demonstrate trapping of custom-synthesized 20 nm nanoparticles based on molecular graphene quantum dots using metamaterial plasmonic tweezers. Superior trap stiffness values as high as 8.8 (fN/nm)/(mW/$\mu\mbox{m}^2$) were achieved with optical intensities lower than 1 mW/$\mu\mbox{m}^2$. By gradually increasing the laser intensity we identified a critical value beyond which the stiffness values dropped significantly. This value corresponded to a temperature rise of about 16$^o$C, evidently sufficient to create thermal flows and disrupt the trapping performance. We, therefore, identified a safe intensity regime for trapping nanoparticles without unwanted heat. Our platform can be used for efficient nanopositioning of fluorescent particles and quantum emitters in an array configuration, potentially acting as a single-photon source configuration.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -cd -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk -cd \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -cd -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -cd -lualatex \"$_[0]\"" );
   }
}
